QFactor: A Domain-Specific Optimizer for Quantum Circuit Instantiation

We introduce a domain-specific algorithm for numerical optimization operations used by quantum circuit instantiation, synthesis, and compilation methods. QFactor uses a tensor network formulation together with analytic methods and an iterative local optimization algorithm to reduce the number of problem parameters. Besides tailoring the optimization process, the formulation is amenable to portable parallelization across CPU and GPU architectures, which is usually challenging in general purpose optimizers (GPO). Compared with several GPOs, our algorithm achieves exponential memory and performance savings with similar optimization success rates. While GPOs can handle directly circuits of up to six qubits, QFactor can process circuits with more than 12 qubits. Within the BQSKit optimization framework, we enable optimizations of 100+ qubit circuits using gate deletion algorithms to scale out linearly with the hardware resources allocated for compilation in GPU environments.

==> sections/inst.tex <==
\section{Parameterized Circuit Instantiation}
\label{sec:inst}

Instantiation is the process of finding the parameters for
a circuit's gates that make it to most closely implement
a target unitary. Techniques that perform instantiation are ubiquitously
deployed in quantum compiler toolchains. The formal problem definition is given by:

\parah{Parameterized Circuit Instantiation Problem}
Given a parameterized quantum circuit $C: \mathbb{R}^k \mapsto U(N)$ and a target
unitary $V \in U(N)$, solve for $$\argmax_{\alpha}{tr(V^{\dagger}C(\alpha))}$$
where $k$ is the number of gate parameters in the circuit, and $U(N)$ is the set of all $N \times N$ unitary matrices. This definition is very general and considers the parameterized circuit as a parameterized unitary operator, see Figure~\ref{fig:params}. The $tr(V^\dagger C(\alpha))$ component measures the Hilbert-Schmidt inner product, which physically represents the overlap between the target unitary and the circuit's operator. The maximum value this can have is equal to $N$ the dimension of the matrix, and this occurs when $C(\alpha)$, the unitary of the circuit with gate parameters $\alpha$, is equivalent to $V$ the target unitary up to a global phase.

\begin{figure}
    \centering
    \includegraphics[scale=1.5]{figures/instantiation-circuit.pdf}
    \caption{\footnotesize \it This is an example of a parameterized quantum circuit on the left. It is composed of three-parameter universal single-qubit rotations and two-qubit CNOT gates. For simulatable circuits, we can represent the circuit by its unitary operator shown on the right, which is calculated by tensor contraction of all of its gates. Furthermore, we can represent parameterized circuits by a parameterized unitary $C(\alpha)$, which can be instantiated to some other unitary $V$ by solving for the parameters $\alpha$ that maximize the overlap of $C(\alpha)$ and $V$. This can be accomplished with analytic methods in specific cases and gradient descent or other numerical methods in the general case. The text describing a parameterized single-qubit rotation will be left out in the other figures; a box on a single wire depicts a generic parameterized single-qubit gate.}
    \label{fig:params}
\end{figure}

The most common form of instantiation is the KAK~\cite{kak} decomposition, which uses analytic methods to produce the two-qubit circuit that implements  any two-qubit unitary. Compilers have used this decomposition to optimize long sequences of operations. This is done by first grouping together consecutive gates on a pair of qubits, then calculating the unitary implemented by the grouped gates, and finally applying the KAK decomposition to convert to a potentially shorter sequence of gates.

For every universal gate-set, the KAK decomposition can yield a parameterized circuit, to which it can instantiate any two-qubit unitary. Therefore, applying the KAK decomposition to retarget a circuit's gate-set is also possible. Once a template is discovered in the desired gate-set, it can be utilized similarly to the optimization procedure to convert grouped gates to gates of a different type. However, producing a circuit template when designing a new gate-set may be nontrivial.

Recently, bottom-up approaches to quantum synthesis have been successful through numerical instantiation~\cite{qsearch, qfast, nacl, squander1, squander2, bestapprox}.
Rather than fixed mathematical identities, these techniques employ a numerical optimizer to closely approximate a solution to the instantiation problem. This is done by minimizing a cost function, often the unitary error or distance between the circuit's unitary and a target unitary. This is given by the following formula using the same notation as before.

$$\Delta(C(\alpha), V) = 1 - \frac{|tr(V^\dagger C(\alpha))|}{N}$$

Other variations of this distance function include:

$$\Delta_f(C(\alpha), V) = 1 - \frac{Re(tr(V^\dagger C(\alpha)))}{N}$$

and

$$\Delta_p(C(\alpha), V) = \sqrt{1 - \frac{|tr(V^\dagger C(\alpha))|^2}{N^2}}$$

All three methods have a range of $[0, 1]$, and as they approach zero, the circuit's
unitary approaches V. For the rest of our paper, we refer to the unitary
distance or error as $\Delta$, the first formulation.

Bottom-up synthesis methods build up the parameterized circuit by iteratively placing more gates. At every step, they instantiate the parameters using numerical optimizers and claim a solution when the error is less than some $\epsilon$ threshold. For example, QSearch~\cite{qsearch} phrases the synthesis problem as a search over circuit templates, instantiating candidates as it searches over them. QFAST~\cite{qfast} expands on this by conflating the search and numerical optimization using a unique circuit encoding. In the NACL~\cite{nacl} algorithm, machine learning methods are used alongside instantiation to synthesize noise-aware circuits. SQUANDER~\cite{squander2} takes a more direct approach to bottom-up synthesis. Here the circuit template is grown and reinstantiated iteratively until a solution is found, at which point, the circuit is then compressed into its optimal form. In~\cite{bestapprox}, instantiation is used in a similar bottom-up approach to produce approximate circuits. More recently, the optimization space of instantiation has been studied and a hypertuned synthesis algorithm, CPFlow~\cite{cpflow}, has been built. Lastly, in Quartz~\cite{quartz}, a similar method to instantiation is employed to dynamically construct circuit substitution rules for any environment.

Several compilation algorithms have leveraged the high quality of results produced during bottom-up synthesis. QGo~\cite{qgo} combined circuit partitioning with synthesis to create a circuit mapping and optimization procedure. QUEST~\cite{quest} uses similar techniques to produce robust and resource-efficient approximate circuits. The growth of algorithms using numerical instantiation has been a motivation for BQSKit~\cite{bqskit} developers to build a Python framework around instantiation.

